Predictive Control for Autonomous Driving with Uncertain, Multi-modal Predictions

We propose a Stochastic MPC (SMPC) formulation for path planning with autonomous vehicles in scenarios involving multiple agents with multi-modal predictions. The multi-modal predictions capture the uncertainty of urban driving in distinct modes/maneuvers (e.g., yield, keep speed) and driving trajectories (e.g., speed, turning radius), which are incorporated for multi-modal collision avoidance chance constraints for path planning. In the presence of multi-modal uncertainties, it is challenging to reliably compute feasible path planning solutions at real-time frequencies ($\geq$ 10 Hz). Our main technological contribution is a convex SMPC formulation that simultaneously (1) optimizes over parameterized feedback policies and (2) allocates risk levels for each mode of the prediction. The use of feedback policies and risk allocation enhances the feasibility and performance of the SMPC formulation against multi-modal predictions with large uncertainty. We evaluate our approach via simulations and road experiments with a full-scale vehicle interacting in closed-loop with virtual vehicles. We consider distinct, multi-modal driving scenarios: 1) Negotiating a traffic light and a fast, tailgating agent, 2) Executing an unprotected left turn at a traffic intersection, and 3) Changing lanes in the presence of multiple agents. For all of these scenarios, our approach reliably computes multi-modal solutions to the path-planning problem at real-time frequencies.

==> Sections/proof.tex <==
\section{Proof of our ADF Policy Class being equivalent to state feedback} 
\subsection*{Setup: Models}
Let the LTV ego vehicle dynamics be given by 
\begin{align}\label{EV_dyn}
    \Delta x_{t+1}=A_t\Delta x_t+B_t\Delta u_t+w_t ~\forall t=0,\dots,N-1
\end{align}
where $w_t\sim\mathcal{N}(0,\Sigma_w)$.  The target vehicle dynamics be given by the switched ATV model
\begin{align}\label{TV_dyn}
    o_{t+1}=T_{t,\sigma_t}o_t+c_{t,\sigma_t}+n_{t}~\forall t=0,\dots, N-1
\end{align}
where $n_{t}\sim\mathcal{N}(0,\Sigma_n)$ and $\sigma_t\in\{1,\dots,J\}$ is the mode at time $t$.
Define the matrices $$\tilde{A}_{t,\sigma_t}=\begin{bmatrix}A_t&O\\O&T_{t,\sigma_t}\end{bmatrix}, \tilde{B}_{t}=\begin{bmatrix}B_t\\O\end{bmatrix}, \tilde{C}_{t,\sigma_t}=\begin{bmatrix}O\\c_{t,\sigma_t}\end{bmatrix}$$and stack the states and disturbances of \eqref{EV_dyn}, \eqref{TV_dyn} as $$\tilde{x}_t=\begin{bmatrix}\Delta x_t\\o_t\end{bmatrix},\ \tilde{w}_{t}=\begin{bmatrix}w_t\\n_{t}\end{bmatrix}.$$

The mode $\sigma_t$ is assumed unknown until some time $\bar t> 0$ in the future.

\begin{assumption}\label{assmp:tbar}
At time $\bar t> 0$, we can determine the mode $\sigma_{\bar t}$ from $o_{\bar t}$ and this mode is fixed for the remaining time steps, i.e., $\sigma_t=\sigma_{\bar t}~\forall t=\bar t, \dots, N-1$.
\end{assumption} 


Denote the mode sequence $\{\sigma_i\}_{i=0}^t$ by $\sigma_0^t$.
Given $\bar t$, define the set of admissible switching sequences as 
\begin{align}
    \mathcal{S}_{\bar t}=\{\hat\sigma_0^{N-1}\in\{1,\dots,J\}^N : \hat\sigma_t=\hat\sigma_{\bar t} ~\forall t\geq \bar t \}.
\end{align}
By assumption \ref{assmp:tbar}, the actual mode sequence $\sigma_0^{N-1}$ lies in this set, i.e., $\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$.


For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, let $\mathbf{x}^{\hat\sigma_0^{N-1}}=[\tilde{x}_0^\top\dots,\tilde{x}_N^\top]^\top$ be the states obtained by applying $\mathbf{u}=[\Delta u_0^\top\dots,\Delta u_{N-1}^\top]^\top$, as given by
\small
\begin{align}\label{eq:states_stacked}
\mathbf{x}^{\hat\sigma_0^{N-1}}=\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}_0+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{u}+\mathbf{C}^{\hat\sigma_0^{N-1}}+\mathbf{E}^{\hat\sigma_0^{N-1}}\mathbf{w}
\end{align}
\normalsize
where $\mathbf{w}=[\tilde{w}_0^\top\dots\tilde{w}_{N-1}^\top]^\top$, 

\scriptsize
\begin{align*}
    &\mathbf{A}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}I\\\tilde{A}_{0,\hat\sigma_0}\\\tilde{A}_{1,\hat\sigma_1}\tilde{A}_{0,\hat\sigma_0}\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{0,\hat\sigma_0}\end{bmatrix},\\
    &\mathbf{C}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O\\\tilde{C}_{0,\hat\sigma_0}\\\tilde{C}_{1,\hat\sigma_1}+\tilde{A}_{1,\hat\sigma_1}\tilde{C}_{0,\hat\sigma_0}\\\vdots\\\tilde{C}_{N-1,\hat\sigma_{N-1}}+\sum_{k=0}^{N-2}\tilde{A}_{N-1,\hat\sigma_{N-1}}\dots \tilde{A}_{k+1,\hat\sigma_{k+1}}\tilde{C}_{k,\hat\sigma_k}\end{bmatrix},\\
    &\mathbf{B}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O&\hdots&\hdots& O\\\tilde{B}_{0}&O&\hdots&O\\\tilde{A}_{1,\hat\sigma_1}\tilde{B}_{0}&\tilde{B}_{1}&\hdots&O\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{1,\hat\sigma_1}\tilde{B}_{0}&\hdots&\tilde{A}_{N-1,\hat\sigma_{N-1}}\tilde{B}_{N-2}&\tilde{B}_{N-1}\end{bmatrix},\\
    &\mathbf{E}^{\hat\sigma_0^{N-1}}=\begin{bmatrix}O&\hdots&\hdots& O\\I&O&\hdots&O\\\tilde{A}_{1,\hat\sigma_1}&I&\hdots&O\\\vdots\\\tilde{A}_{N-1,\hat\sigma_{N-1}}\hdots\tilde{A}_{1,\hat\sigma_1}&\hdots&\tilde{A}_{N-1,\hat\sigma_{N-1}}&I\end{bmatrix}.
\end{align*}
\normalsize
\subsection*{Setup: Control Problem}
Given initial condition $\tilde{x}_0=\tilde{x}$, we seek feedback policies $\Delta u_t=\pi_t(\tilde{x}_t)~\forall t=0,\dots,N-1$ such that the following 
 obstacle avoidance constraints and input constraints are  satisfied by \eqref{EV_dyn}, \eqref{TV_dyn}: 
\begin{align}
    &\mathbb{P}(\mathbf{H}\mathbf{x}^{\sigma_0^{N-1}}\leq \mathbf{h}\ |\tilde{x}_0=\tilde{x} )\geq p,\\
    &\mathbb{P}(\mathbf{G}\mathbf{u}^{\sigma_0^{N-1}}\leq \mathbf{g}\ |\tilde{x}_0=\tilde{x})\geq p
\end{align}
where $\mathbf{u}^{\sigma_0^{N-1}}=[\pi_0(\tilde{x}_0)^\top\dots\pi_{N-1}(\tilde{x}_{N-1})^\top]^\top$ and $\mathbf{H}, \mathbf{G}$ have $n_H$ and $n_G$ rows respectively. 
Note that $\sigma_0^{N-1}$ is not known at $t=0$, and thus we look for policies $\pi_t(\cdot)$ such that
\begin{align}\label{control_problem}
    &\mathbb{P}(\mathbf{H}\mathbf{x}^{\hat\sigma_0^{N-1}}\leq \mathbf{h}\ |\tilde{x}_0=\tilde{x} )\geq p,\nonumber\\
    &\mathbb{P}(\mathbf{G}\mathbf{u}^{\hat\sigma_0^{N-1}}\leq \mathbf{g}\ |\tilde{x}_0=\tilde{x})\geq p~~ \forall\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}.
\end{align}
\subsection*{Policy Candidates}
\subsubsection{Affine state feedback policy class}

Consider the following control policy
\small
\begin{align}\label{eq:ASF}
    \pi^{ASF}_{t}(\tilde{x}_t)=\begin{cases}
    \sum_{k=0}^tK_{k,t}\tilde{x}_k+v_t, &\text{for } t<\bar t\\
    \sum_{k=0}^tK^{1}_{k,t}\tilde{x}_k+v^{1}_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=1\\
    \vdots & \vdots\\
    \sum_{k=0}^tK^{J}_{k,t}\tilde{x}_k+v^{J}_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=J
    \end{cases}
\end{align}
\normalsize
In view of assumption \ref{assmp:tbar}, this policy is mode-agnostic for $t<\bar t$ and mode-dependent for $t\geq \bar t$.
For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, define 
\scriptsize
$$\mathbf{v}^{\hat\sigma_{\bar t}}=[v_0^\top\dots v_{\bar t-1}^\top\  v^{\hat\sigma_{\bar t}\top}_{\bar t}\dots v^{\hat\sigma_{\bar t}\top}_{N-1}]^\top, $$
\begin{align*}
    \mathbf{K}^{\hat\sigma_{\bar t}}=\begin{bmatrix}K_{0,0}&O&\hdots&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K_{0,\bar t-1}&\hdots K_{\bar t-1,\bar t-1}&O&\hdots& O\\
    K^{\hat\sigma_{\bar t}}_{0,\bar t}&\hdots &K^{\hat\sigma_{\bar t}}_{\bar t,\bar t}&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K^{\hat\sigma_{\bar t}}_{0,N-1}&\hdots &\hdots& K^{\hat\sigma_{\bar t}}_{N-1,N-1}&O
    \end{bmatrix}
\end{align*}
\normalsize
to get 
\begin{align}\label{eq:ASF_control_stacked}
\mathbf{u}_{ASF}^{\hat\sigma_0^{N-1}}=\mathbf{K}^{\hat\sigma_{\bar t}}\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}+\mathbf{v}^{\hat\sigma_{\bar t}}.
\end{align}
where $\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}$ is the closed-loop trajectory given by substituting \eqref{eq:ASF_control_stacked} in \eqref{eq:states_stacked}. The closed-loop trajectory can be given in closed-form as 
\small
\begin{align}\label{eq:ASF_stacked_states}
    \mathbf{x}^{\hat\sigma_0^{N-1}}_{ASF}=&(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}_0+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})\nonumber\\&+(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\mathbf{w}
\end{align}
\normalsize
where the matrix $\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}}$ can be shown to be lower triangular with all diagonal entries being $1$, and thus, invertible. Note that due to the presence of the inverse $(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}$, the closed-loop states $\mathbf{x}^{\hat\sigma_0^{N-1}}_{ASF}$ are generally nonlinear functions of $\mathbf{K}^{\hat\sigma_{\bar t}},\ \mathbf{v}^{\hat\sigma_{\bar t}}$. 


For given $\hat\sigma_0^{N-1}$ and $ \mathbf{K}^{\hat\sigma_{\bar t}}, \mathbf{v}^{\hat\sigma_{\bar t}}$, the chance constraints \eqref{control_problem} can be tightened as follows. 
\footnotesize
\begin{align}\label{state_chance_constr_tightened}
    &\mathbb{P}(\mathbf{H}_i\mathbf{x}_{ASF}^{\hat\sigma_0^{N-1}}>\mathbf{h}_i |\tilde{x}_0=\tilde{x})\leq\frac{1-p}{n_H}~\forall i=1,\dots,n_H\nonumber\\
    \Leftrightarrow&\mathbf{H}_i(\mathbf{I}-\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})\nonumber\\
    &~~+\text{cdf}^{-1}\left(p_H\right)\Vert\mathbf{H}_i(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\Sigma_{\tilde{w}}^{\frac{1}{2}}\Vert\leq\mathbf{h}_i\nonumber\\
    &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\forall i=1,\dots,n_H
\end{align}
\begin{align}\label{input_chance_constr_tightened}
    &\mathbb{P}(\mathbf{G}_j\mathbf{u}_{ASF}^{\hat\sigma_0^{N-1}}>\mathbf{g}_j|\tilde{x}_0=\tilde{x})\leq\frac{1-p}{n_G}~\forall j=1,\dots,n_G\nonumber\\
    \Leftrightarrow&\mathbf{G}_j(\mathbf{K}^{\hat\sigma_{\bar t}}(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}(\mathbf{A}^{\hat\sigma_0^{N-1}}\tilde{x}+\mathbf{B}^{\hat\sigma_0^{N-1}}\mathbf{v}^{\hat\sigma_{\bar t}}+\mathbf{C}^{\hat\sigma_0^{N-1}})+\mathbf{v}^{\hat\sigma_{\bar t}})\nonumber\\&~~+\text{cdf}^{-1}\left(p_G\right)\Vert\mathbf{G}_j\mathbf{K}^{\hat\sigma_{\bar t}}(\mathbf{I}-\mathbf{B}^\mathbf{K}^{\hat\sigma_{\bar t}})^{-1}\mathbf{E}^{\hat\sigma_0^{N-1}}\Sigma_{\tilde{w}}^{\frac{1}{2}}\Vert\leq\mathbf{g}_j\nonumber\\
    &~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\forall j=1,\dots,n_G
\end{align}
\normalsize
where cdf$^{-1}(\cdot)$ is the inverse of the cumulative distribution function of $\mathcal{N}(0,1)$, $p_H=1-\frac{1-p}{n_H}$, $p_G=1-\frac{1-p}{n_G}$ and $\Sigma_{\tilde{w}}=\begin{bmatrix}\Sigma_w&O\\O&\Sigma_n\end{bmatrix}$.


For a given initial condition $\tilde{x}_0=\tilde{x}$, an inner approximation of the class of affine state feedback policies of the form \eqref{eq:ASF} that satisfies \eqref{control_problem} is given by the set
\begin{align}
    \Pi_{ASF}(\tilde{x})=\{\{\mathbf{K}^j,\mathbf{v}^j\}_{\forall j\in\{1,\dots,J\}}:\eqref{state_chance_constr_tightened},\eqref{input_chance_constr_tightened}~ \forall \hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}\ \}
\end{align}
\subsubsection{Affine switched disturbance feedback policy class:}
For any $\hat\sigma_{0}^{N-1}\in\mathcal{S}_{\bar t}$ and any $t\geq 1$, we can use measurements $\tilde{x}_t, \tilde{x}_{t-1}$ and $\Delta u_{t-1}$ to define $$\tilde{w}_{t-1,\hat\sigma_{t-1}}=\tilde{x}_{t}-\tilde{A}_{t-1,\hat\sigma_{t-1}}\tilde{x}_{t-1}-\tilde{B}_{t-1}\Delta u_{t-1}-\tilde{C}_{t-1,\hat\sigma_{t-1}}.$$ 
 For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, let
\small
\begin{align}\label{eq:ADF_sigma}
    &u^{\hat\sigma_0^{N-1}}_{t}=\begin{cases}
    \sum_{k=0}^{t-1}M_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h_t, &\text{for } t<\bar t\\
    M^1_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h^1_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=1\\
    \vdots & \vdots\\
    M^J_{k,t}\begin{bmatrix}w_{k}\\n_{k,\hat\sigma_k}\end{bmatrix}+h^J_t, &\text{for } t\geq\bar t,\ \sigma_{\bar t}=J
    \end{cases}
\end{align}
\normalsize
and define the feedback control policy as
\begin{align}\label{eq:ADF}
    \pi^{ASDF}(\tilde{x}_t)\in\{u^{\hat\sigma_0^{N-1}}_{t}\}_{\forall\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}}
\end{align}
Like \eqref{eq:ASF}, this policy is mode agnostic for $t<\bar t$ and mode-dependent for $t\geq \bar t$. However, this policy is non-deterministic except at $t=0$ when $\pi^{ASDF}_0(\tilde{x}_0)=h_0$.

For any $\hat\sigma_0^{N-1}\in\mathcal{S}_{\bar t}$, define 
\scriptsize
$$\mathbf{h}^{\hat\sigma_{\bar t}}=[h_0^\top\dots h_{\bar t-1}^\top\  h^{\hat\sigma_{\bar t}\top}_{\bar t}\dots h^{\hat\sigma_{\bar t}\top}_{N-1}]^\top, $$
\begin{align*}
    \mathbf{M}^{\hat\sigma_{\bar t}}=\begin{bmatrix}
    O&\hdots&\hdots&\hdots& O\\M_{0,1}&O&\hdots&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K_{0,\bar t-1}&\hdots K_{\bar t-1,\bar t-1}&O&\hdots& O\\
    K^{\hat\sigma_{\bar t}}_{0,\bar t}&\hdots &K^{\hat\sigma_{\bar t}}_{\bar t,\bar t}&\hdots& O\\
    \vdots&\vdots&\vdots&\vdots\\
    K^{\hat\sigma_{\bar t}}_{0,N-1}&\hdots &\hdots& K^{\hat\sigma_{\bar t}}_{N-1,N-1}&O
    \end{bmatrix}
\end{align*}
\normalsize

